Cybersecurity Discussions in Stack Overflow: A Developer-Centred Analysis of Engagement and Self-Disclosure Behaviour

Stack Overflow (SO) is a popular platform among developers seeking advice on various software-related topics, including privacy and security. As for many knowledge-sharing websites, the value of SO depends largely on users' engagement, namely their willingness to answer, comment or post technical questions. Still, many of these questions (including cybersecurity-related ones) remain unanswered, putting the site's relevance and reputation into question. Hence, it is important to understand users' participation in privacy and security discussions to promote engagement and foster the exchange of such expertise. Objective: Based on prior findings on online social networks, this work elaborates on the interplay between users' engagement and their privacy practices in SO. Particularly, it analyses developers' self-disclosure behaviour regarding profile visibility and their involvement in discussions related to privacy and security. Method: We followed a mixed-methods approach by (i) analysing SO data from 1239 cybersecurity-tagged questions along with 7048 user profiles, and (ii) conducting an anonymous online survey (N=64). Results: About 33% of the questions we retrieved had no answer, whereas more than 50% had no accepted answer. We observed that "proactive" users tend to disclose significantly less information in their profiles than "reactive" and "unengaged" ones. However, no correlations were found between these engagement categories and privacy-related constructs such as Perceived Control or General Privacy Concerns. Implications: These findings contribute to (i) a better understanding of developers' engagement towards privacy and security topics, and (ii) to shape strategies promoting the exchange of cybersecurity expertise in SO.

==> card_sorting.tex <==
\newpage
\thispagestyle{empty}

\section*{Disclosure of Display Names and Locations (card sorting)}
\textit{Display names} in SO are kept separately from the real private name. While the former is publicly shown in the network, the latter is used only on SO-directed job applications and remains inaccessible through the StackExchange API. \textit{Locations} are also presented as text fields allowing users to obfuscate this information (e.g., put their country instead of the city) or even write whatever they want. We conducted a card-sorting analysis to determine the reliability of these two fields (and of the proposed coding schema).

Card sorting is a frequently used technique to derive taxonomies and prevent biases when categorising data. During a card sorting iteration, a person organises entities into a set of prefixed categories based on some common criterion. Once two or more people conduct this process, classification disagreements are discussed and resolved consensually. Here, each author performed a single card sorting iteration (i.e., one for display names and one for locations) using the following classification rules:

\begin{itemize}
\item \textit{Display names} were categorised as \textbf{1} in case of full real names, \textbf{0.5} for partial or shortened real names, and \textbf{0} in the case of fantasy names. 
\item \textit{Locations} were classified as \textbf{1} when including a ZIP/Postal code, \textbf{0.66} for cities or states, \textbf{0.33} for countries or large regions (e.g., Europe), and \textbf{0} in case of fictitious places.
\end{itemize}

We conducted such an analysis over a generalisable sample of locations and display names using a confidence level of 95\%. Since \textit{display names} are mandatory, we generated a sample of 374 names from a population of 3574. On the other hand, we sampled 329 locations out of a total of 2248 (we only considered those that were not empty). Both samples were randomly selected using an R script.

Once each author had sorted the samples, we applied Cohen's Kappa coefficient to compute the inter-rater reliability of both classifications. Cohen's Kappa measures the level of agreement between two or more raters responsible for sorting items into mutually exclusive categories. A value closer to $+1$ suggests a high inter-rater agreement, whereas a value approaching $-1$ would indicate a high disagreement among raters. We adopted an agreement/disagreement threshold of $0.79$ according to common practices and conventions for its adequate interpretation. 

The coefficients obtained in both cases ($+0.80$ for \textit{display names} and $+0.86$ for \textit{locations}) indicate a high rate of agreement and reliability of the corresponding coding schemas. Moreover, after completing the card sorting analysis, 55\% of the \textit{display names} had been classified as full or partially-full real names, and 97\% of locations as cities, states, countries, or large regions. \textbf{Hence, we concluded that when such information is present in a SO profile, it can be considered accurate.}
